The RQR algorithm

Pole-swapping algorithms, generalizations of bulge-chasing algorithms, have been shown to be a viable alternative to the bulge-chasing QZ algorithm for solving the generalized eigenvalue problem for a matrix pencil A - {\lambda}B. It is natural to try to devise a pole-swapping algorithm that solves the standard eigenvalue problem for a single matrix A. This paper introduces such an algorithm and shows that it is competitive with Francis's bulge-chasing QR algorithm.

==> bwe.tex <==
\addplot[%
    SPECred,%
    mark=square*,%
    mark options = {solid, fill = SPECred},%
 ]coordinates{%
  (1,1.304240e-15)%
  (2,1.613658e-15)%
  (3,1.997408e-15)%
  (4,2.423353e-15)%
  (5,2.965546e-15)%
  (6,3.594462e-15)%
  (7,4.360734e-15)%
  (8,5.312283e-15)%
  (9,6.445350e-15)%
  (10,7.780474e-15)%
  (11,9.437730e-15)%
  (12,1.148256e-14)%
  (13,1.398692e-14)%
};%
\addplot[%
    SPECblue,%
    mark=square*,%
    mark options = {solid, fill = SPECblue},%
 ]coordinates{%
  (1,1.930508e-15)%
  (2,2.420474e-15)%
  (3,3.027805e-15)%
  (4,3.697346e-15)%
  (5,4.546695e-15)%
  (6,5.539266e-15)%
  (7,6.746725e-15)%
  (8,8.405769e-15)%
  (9,1.057951e-14)%
  (10,1.245007e-14)%
  (11,1.527723e-14)%
  (12,1.932054e-14)%
  (13,2.535456e-14)%
};%
\addplot[%
    SPECred,%
    dashed,%
    mark=o*,%
    mark options = {solid, fill = SPECred},%
 ]coordinates{%
  (1,8.612518e-16)%
  (2,1.000025e-15)%
  (3,1.433867e-15)%
  (4,1.386756e-15)%
  (5,1.872672e-15)%
  (6,2.467562e-15)%
  (7,2.954526e-15)%
  (8,3.895035e-15)%
  (9,4.971063e-15)%
  (10,5.851678e-15)%
  (11,7.845624e-15)%
  (12,9.075919e-15)%
  (13,1.564504e-14)%
};%
\addplot[%
    SPECblue,%
    dashed,%
    mark=o*,%
    mark options = {solid, fill = SPECblue},%
 ]coordinates{%
  (1,2.057502e-15)%
  (2,2.032744e-15)%
  (3,2.558498e-15)%
  (4,3.197796e-15)%
  (5,4.649990e-15)%
  (6,5.409763e-15)%
  (7,6.396101e-15)%
  (8,8.814569e-15)%
  (9,1.017827e-14)%
  (10,1.182752e-14)%
  (11,1.373809e-14)%
  (12,1.370656e-14)%
  (13,2.072984e-14)%
};%


==> bwe_ratio.tex <==
\addplot[%
    black,%
    mark=square*,%
    mark options = {solid, fill = black},%
 ]coordinates{%
  (1,6.755939e-01)%
  (2,6.666703e-01)%
  (3,6.596885e-01)%
  (4,6.554305e-01)%
  (5,6.522423e-01)%
  (6,6.489058e-01)%
  (7,6.463483e-01)%
  (8,6.319806e-01)%
  (9,6.092296e-01)%
  (10,6.249340e-01)%
  (11,6.177646e-01)%
  (12,5.943188e-01)%
  (13,5.516530e-01)%
};%
\addplot[%
    black,%
    dashed,%
    %mark=*,%
    mark options = {solid, fill = black},%
 ]coordinates{%
  (1,4.185910e-01)%
  (2,4.919584e-01)%
  (3,5.604332e-01)%
  (4,4.336600e-01)%
  (5,4.027260e-01)%
  (6,4.561313e-01)%
  (7,4.619261e-01)%
  (8,4.418860e-01)%
  (9,4.883994e-01)%
  (10,4.947509e-01)%
  (11,5.710854e-01)%
  (12,6.621586e-01)%
  (13,7.547110e-01)%
};%


==> runtime.tex <==
\addplot[%
    SPECred,%
    mark=square*,%
    mark options = {solid, fill = SPECred},%
 ]coordinates{%
  (1,3.880602e-05)%
  (2,8.740866e-05)%
  (3,2.138661e-04)%
  (4,5.146575e-04)%
  (5,1.347000e-03)%
  (6,3.543103e-03)%
  (7,1.012192e-02)%
  (8,3.298636e-02)%
  (9,1.627400e-01)%
  (10,5.034600e-01)%
  (11,1.088850e+00)%
  (12,3.586290e+00)%
  (13,1.551273e+01)%
};%
\addplot[%
    SPECblue,%
    mark=square*,%
    mark options = {solid, fill = SPECblue},%
 ]coordinates{%
  (1,4.406617e-05)%
  (2,1.021786e-04)%
  (3,2.572907e-04)%
  (4,6.249315e-04)%
  (5,1.665846e-03)%
  (6,4.523448e-03)%
  (7,1.322538e-02)%
  (8,4.566182e-02)%
  (9,2.250020e-01)%
  (10,6.826900e-01)%
  (11,1.613100e+00)%
  (12,5.411180e+00)%
  (13,2.229600e+01)%
};%
\addplot[%
    SPECred,%
    dashed,%
    mark=o*,%
    mark options = {solid, fill = SPECred},%
 ]coordinates{%
  (1,3.621654e-05)%
  (2,7.630582e-05)%
  (3,1.941705e-04)%
  (4,4.728767e-04)%
  (5,1.226692e-03)%
  (6,3.382414e-03)%
  (7,9.433077e-03)%
  (8,3.168818e-02)%
  (9,1.597660e-01)%
  (10,4.811850e-01)%
  (11,1.012860e+00)%
  (12,3.238760e+00)%
  (13,1.593003e+01)%
};%
\addplot[%
    SPECblue,%
    dashed,%
    mark=o*,%
    mark options = {solid, fill = SPECblue},%
 ]coordinates{%
  (1,5.020752e-05)%
  (2,1.074966e-04)%
  (3,2.684170e-04)%
  (4,6.315411e-04)%
  (5,1.514692e-03)%
  (6,4.399483e-03)%
  (7,1.254846e-02)%
  (8,4.547636e-02)%
  (9,2.006700e-01)%
  (10,6.062600e-01)%
  (11,1.464010e+00)%
  (12,5.150250e+00)%
  (13,1.830334e+01)%
};%


==> runtime_ratio.tex <==
\addplot[%
    black,%
    mark=square*,%
    mark options = {solid, fill = black},%
 ]coordinates{%
  (1,8.806306e-01)%
  (2,8.554496e-01)%
  (3,8.312234e-01)%
  (4,8.235423e-01)%
  (5,8.085981e-01)%
  (6,7.832749e-01)%
  (7,7.653405e-01)%
  (8,7.224058e-01)%
  (9,7.232825e-01)%
  (10,7.374650e-01)%
  (11,6.750046e-01)%
  (12,6.627556e-01)%
  (13,6.957629e-01)%
};%
\addplot[%
    black,%
    dashed,%
    %mark=*,%
    mark options = {solid, fill = black},%
 ]coordinates{%
  (1,7.213370e-01)%
  (2,7.098439e-01)%
  (3,7.233910e-01)%
  (4,7.487663e-01)%
  (5,8.098624e-01)%
  (6,7.688208e-01)%
  (7,7.517317e-01)%
  (8,6.968055e-01)%
  (9,7.961629e-01)%
  (10,7.936941e-01)%
  (11,6.918395e-01)%
  (12,6.288549e-01)%
  (13,8.703343e-01)%
};%

